A shifted interface approach for internal discontinuities in poroelastic media

Porous media containing cracks, fractures, or internal discontinuities arise throughout subsurface geomechanics, biomechanics, and materials science. Numerical simulation of the coupled hydromechanical response is inherently challenging because the pressure and displacement fields are tightly coupled through the Biot equations, requiring stable mixed formulations. These difficulties are compounded when cracks are present, because standard mesh-conforming approaches require costly, labor-intensive, body-fitted meshing, while unfitted methods often require cut-cell integration, enrichment functions, or additional stabilization. In this work, we use an alternative approach, we adapt the shifted interface method to coupled transient poroelasticity with embedded interfaces. The method replaces the true crack by a surrogate approximation where interface conditions are transferred through local expansions. A unified derivation yields shifted forms for both hydraulic transmission and mechanical traction coupling. Two enforcement strategies are extensively compared: a weak (integral) enforcement and a strong (pointwise) enforcement. Four test cases of increasing geometric complexity (offset mesh-aligned, boundary-intersecting angled, embedded angled, and multi-crack configurations) validate the formulation. Away from crack tips, interface residuals converge as O(h); near tips, localized post-processing artifacts degrade the global rate, but first-order convergence is recovered when a small tip region is excluded. A multi-crack demonstration with four simultaneously embedded cracks of distinct geometry and interface properties confirms the practical applicability of the framework. These results support the shifted interface method as a practical framework for poroelastic crack modeling on non-body-fitted meshes with geometrically complex embedded interfaces.

==> figures/30_angle/convergence_table.tex <==
\begin{table}[htbp]
\centering
\caption{Convergence of interface residual $L^2$ norms for the
$30^\circ$ angled crack. The flow constitutive and flux balance
residuals are indistinguishable between the two enforcement strategies
and are listed once; the traction balance and constitutive residuals
differ and are reported separately for the nodal and weak strategies.
Residuals are defined
in~\cref{eq:balance_residuals,eq:constitutive_residual_flow,eq:constitutive_residual_mech}.}
\label{tab:convergence_30angle}
\begin{tabular}{cccccccccccc}
\toprule
& & & &
\multicolumn{2}{c}{$\|r_i^{\jmp{t}}\hat{n}_i\|$} &
\multicolumn{2}{c}{$\|r_i^{\jmp{t}}\hat{m}_i\|$} &
\multicolumn{2}{c}{$\|r_i^{\mathsf{T}}\hat{n}_i\|$} &
\multicolumn{2}{c}{$\|r_i^{\mathsf{T}}\hat{m}_i\|$} \\
\cmidrule(lr){5-6}\cmidrule(lr){7-8}\cmidrule(lr){9-10}\cmidrule(lr){11-12}
$n$ & $h$
& $\|r^{\mathsf{J}}\|$
& $\|r^{\jmp{q}}\|$
& nodal & weak & nodal & weak & nodal & weak & nodal & weak \\
\midrule
 20 & 0.0500 & 1.26e-07 & 2.52e-07 & 9.92e-02 & 5.73e-02 & 9.53e-02 & 5.78e-02 & 3.82e-02 & 1.51e+00 & 9.26e-02 & 1.68e+00 \\
 40 & 0.0250 & 1.01e-07 & 2.01e-07 & 3.77e-02 & 3.49e-02 & 5.42e-02 & 3.47e-02 & 1.69e-02 & 3.90e-01 & 5.25e-02 & 6.23e-01 \\
 80 & 0.0125 & 7.69e-08 & 1.54e-07 & 2.01e-02 & 1.45e-02 & 1.63e-02 & 1.37e-02 & 8.31e-03 & 9.41e-02 & 1.04e-02 & 9.88e-02 \\
160 & 0.0063 & 6.31e-08 & 1.26e-07 & 9.71e-03 & 7.17e-03 & 7.97e-03 & 6.79e-03 & 3.98e-03 & 2.20e-02 & 4.86e-03 & 2.61e-02 \\
\bottomrule
\end{tabular}
\end{table}


==> figures/30_angle_sub/convergence_table.tex <==
\begin{table}[htbp]
\centering
\caption{Convergence of interface residual $L^2$ norms for the
embedded $30^\circ$ angled crack. The flow constitutive and flux
balance residuals are indistinguishable between the two enforcement
strategies and are listed once; the traction balance and constitutive
residuals differ and are reported separately for the nodal and weak
strategies. Non-monotone entries (marked~$\dagger$) are caused by
tip effects discussed in~\cref{sec:embedded_convergence}.
Residuals are defined
in~\cref{eq:balance_residuals,eq:constitutive_residual_flow,eq:constitutive_residual_mech}.}
\label{tab:convergence_embedded}
\begin{tabular}{cccccccccccc}
\toprule
& & & &
\multicolumn{2}{c}{$\|r_i^{\jmp{t}}\hat{n}_i\|$} &
\multicolumn{2}{c}{$\|r_i^{\jmp{t}}\hat{m}_i\|$} &
\multicolumn{2}{c}{$\|r_i^{\mathsf{T}}\hat{n}_i\|$} &
\multicolumn{2}{c}{$\|r_i^{\mathsf{T}}\hat{m}_i\|$} \\
\cmidrule(lr){5-6}\cmidrule(lr){7-8}\cmidrule(lr){9-10}\cmidrule(lr){11-12}
$n$ & $h$
& $\|r^{\mathsf{J}}\|$
& $\|r^{\jmp{q}}\|$
& nodal & weak & nodal & weak & nodal & weak & nodal & weak \\
\midrule
 20 & 0.0500 & 8.24e-07 & 6.71e-07 & 3.89e-02 & 3.70e-02 & 6.31e-02 & 5.32e-02 & 2.48e-02 & 1.29e+00 & 5.42e-02 & 1.95e+00 \\
 40 & 0.0250 & 4.53e-07 & 9.13e-07 & 3.40e-02 & 2.24e+00$^\dagger$ & 4.71e-02 & 5.80e-01$^\dagger$ & 1.82e-02 & 1.17e+01$^\dagger$ & 3.82e-02 & 9.89e-01$^\dagger$ \\
 80 & 0.0125 & 3.14e-07 & 8.70e-07 & 1.49e-02 & 1.69e-02 & 2.05e-02 & 1.77e-02 & 8.50e-02$^\dagger$ & 1.43e-01 & 9.46e-02$^\dagger$ & 1.05e-01 \\
160 & 0.0063 & 8.69e-07 & 6.74e-07 & 4.77e-03 & 1.08e-02 & 8.03e-03 & 7.39e-03 & 7.01e-03 & 2.63e-02 & 1.00e-02 & 4.68e-02 \\
\bottomrule
\end{tabular}
\end{table}


==> figures/aligned_offset/convergence_table.tex <==
\begin{table}[htbp]
\centering
\caption{Convergence of interface residual $L^2$ norms for the mesh-aligned offset crack.
The flow constitutive, flux balance, and traction balance norms are
indistinguishable between the two enforcement strategies (relative differences
below $10^{-2}$) and are listed once; the constitutive residuals
$\|r_i^{\mathsf{T}}\hat{n}_i\|$, $\|r_i^{\mathsf{T}}\hat{m}_i\|$ differ and
are reported separately for the nodal and weak strategies. Residuals are defined
in~\cref{eq:balance_residuals,eq:constitutive_residual_flow,eq:constitutive_residual_mech}.}
\label{tab:convergence_aligned_offset}
\begin{tabular}{cccccccccc}
\toprule
& & & & & & \multicolumn{2}{c}{$\|r_i^{\mathsf{T}}\hat{n}_i\|$} & \multicolumn{2}{c}{$\|r_i^{\mathsf{T}}\hat{m}_i\|$} \\
\cmidrule(lr){7-8}\cmidrule(lr){9-10}
$n$ & $h$
& $\|r^{\mathsf{J}}\|$
& $\|r^{\jmp{q}}\|$
& $\|r_i^{\jmp{t}}\hat{n}_i\|$
& $\|r_i^{\jmp{t}}\hat{m}_i\|$
& nodal & weak & nodal & weak \\
\midrule
 20 & 0.0500 & 1.63e-07 & 3.25e-07 & 1.36e-01 & 4.04e-02 & 1.00e-02 & 3.00e-01 & 3.03e-02 & 1.26e-01 \\
 40 & 0.0250 & 7.09e-08 & 1.42e-07 & 6.95e-02 & 2.12e-02 & 1.97e-03 & 8.58e-03 & 1.44e-02 & 1.83e-02 \\
 80 & 0.0125 & 3.54e-08 & 7.09e-08 & 3.65e-02 & 1.07e-02 & 5.94e-04 & 3.92e-03 & 6.71e-03 & 8.96e-03 \\
160 & 0.0063 & 1.77e-08 & 3.55e-08 & 1.88e-02 & 5.34e-03 & 1.79e-04 & 1.90e-03 & 3.07e-03 & 4.29e-03 \\
\bottomrule
\end{tabular}
\end{table}

